Learning Functional Priors and Posteriors from Data and Physics

We develop a new Bayesian framework based on deep neural networks to be able to extrapolate in space-time using historical data and to quantify uncertainties arising from both noisy and gappy data in physical problems. Specifically, the proposed approach has two stages: (1) prior learning and (2) posterior estimation. At the first stage, we employ the physics-informed Generative Adversarial Networks (PI-GAN) to learn a functional prior either from a prescribed function distribution, e.g., Gaussian process, or from historical data and physics. At the second stage, we employ the Hamiltonian Monte Carlo (HMC) method to estimate the posterior in the latent space of PI-GANs. In addition, we use two different approaches to encode the physics: (1) automatic differentiation, used in the physics-informed neural networks (PINNs) for scenarios with explicitly known partial differential equations (PDEs), and (2) operator regression using the deep operator network (DeepONet) for PDE-agnostic scenarios. We then test the proposed method for (1) meta-learning for one-dimensional regression, and forward/inverse PDE problems (combined with PINNs); (2) PDE-agnostic physical problems (combined with DeepONet), e.g., fractional diffusion as well as saturated stochastic (100-dimensional) flows in heterogeneous porous media; and (3) spatial-temporal regression problems, i.e., inference of a marine riser displacement field. The results demonstrate that the proposed approach can provide accurate predictions as well as uncertainty quantification given very limited scattered and noisy data, since historical data could be available to provide informative priors. In summary, the proposed method is capable of learning flexible functional priors, and can be extended to big data problems using stochastic HMC or normalizing flows since the latent space is generally characterized as low dimensional.

==> 2Dflow.tex <==


\subsection{DeepONet: 2D Flow in heterogeneous porous media}

A two-dimensional flow through heterogeneous porous media is considered here, which is governed by the following equation:
\begin{align}
    \nabla \cdot \left( K(\bm{x}) \nabla h(\bm{x})\right) = 0, ~ \bm{x} = (x, y), ~x, y \in [0, 1],
\end{align}
with boundary conditions:
\begin{align}
    h(0, y) &= 1, ~ h(1, y) = 0, \\
    \partial_{\bm{n}} h(x, 0) &= \partial_{\bm{n}} h(x, 1) = 0,
\end{align}
where $K$ is the hydraulic conductivity, and $h$ is the hydraulic head. Generally, $K$ is determined by the pore structure. To take different structures into consideration, we can then employ a stochastic process to describe $K$. Here we assume that $K = \exp(F(\bm(x)))$, where $F(\bm{x})$ is a truncated Karhunen-Lo\`eve (KL) expansion for a certain Gaussian process, is a widely used model to mimic the real conductivity field, which will also be utilized here. In particular, we keep the leading 100 terms in the KL expansion for the Gaussian process with zero mean and the following kernel:
\begin{align}
    \mathcal{K}(\bm{x}, \bm{x}') = \exp\left[\frac{-(x - x')}{2l^2_1} + \frac{-(y - y')^2} {2 l^2_2} \right],  ~ l_1 = l_2 = 0.25.
\end{align}



\begin{figure}[H]
    \centering
    \subfigure[]{\label{fig:onet_2da}
    \includegraphics[width = 0.9\textwidth]{./Figures/per_2d.png}}
    \subfigure[]{\label{fig:onet_2db}
    \includegraphics[width = 0.9\textwidth]{./Figures/onet_2d.png}}
    \caption{
    (a) Four representative samples for the conductivity field. 
    (b) Predicted $K$ and $h$ with uncertainties. error: $|\psi - \psi^*|$, where $\psi$ represent predicted means of any variables (e.g., $\log(K)$, $h$, etc); $\psi^*$ denotes the exact value; std: standard deviation. Magenta dots: training data for K at the testing stage; Magenta cross: training data for u at the testing stage. 
    }\label{fig:onet_2d}
\end{figure}


We generate data for pretraining with the above truncated KL expansion with a resolution $20 \times 20$ uniform grid. Specifically, 30,000 pairs of $(K, h)$ are generated to train the GANs as well as the DeepONets. On the completion of the training, we assume that we have 10 random noisy measurements on both $K$ and $h$ (Fig. \ref{fig:onet_2d}), and the noise scales for both $K$ and $h$ are the same, i.e., $\mathcal{N}(0, 0.05^2)$. The objective is then to infer $K$ and $h$ in the whole field with uncertainties. The predicted $K$ and $h$ are depicted in Fig. \ref{fig:onet_2d}, we can see: (1) the computational errors between the predicted means and exact solutions for both $K$ and $h$ are bounded by the two standard deviations, and (2) the predicted uncertainties increase for locations without no measurements as expected. 




